BiSHop: Bi-Directional Cellular Learning for Tabular Data with Generalized Sparse Modern Hopfield Model

We introduce the \textbf{B}i-Directional \textbf{S}parse \textbf{Hop}field Network (\textbf{BiSHop}), a novel end-to-end framework for deep tabular learning. BiSHop handles the two major challenges of deep tabular learning: non-rotationally invariant data structure and feature sparsity in tabular data. Our key motivation comes from the recent established connection between associative memory and attention mechanisms. Consequently, BiSHop uses a dual-component approach, sequentially processing data both column-wise and row-wise through two interconnected directional learning modules. Computationally, these modules house layers of generalized sparse modern Hopfield layers, a sparse extension of the modern Hopfield model with adaptable sparsity. Methodologically, BiSHop facilitates multi-scale representation learning, capturing both intra-feature and inter-feature interactions, with adaptive sparsity at each scale. Empirically, through experiments on diverse real-world datasets, we demonstrate that BiSHop surpasses current SOTA methods with significantly less HPO runs, marking it a robust solution for deep tabular learning.

==> 2theory.tex <==
In this section, we generalize the Gini entropic regularizer in Sparsemax-based Hopfield model, i.e. $\Psi(\bp)\coloneqq \half \sum_\nu^M p_\nu(1-p_\nu)$, as Tsallis $\alpha$-entropies \cite{tsallis1988possible} $\Phi(\bp)\coloneqq \frac{1}{\alpha(\alpha-1)}\sum_\nu^M (\bp_\nu-\bp_\nu^\alpha)$, where $\alpha \geq 1$ represents the sparsity.
Based on the convex conjugate of the generalized entropic regularizer, we propose a generalized sparse Hopfield energy and sparse retrieval dynamics to analyze the sparsity-induced properties in the modern Hopfield model.

\subsection{Convergence of Generalized Sparse Hopfield Energy}

In order to discuss the sparsity-dependent properties, we inherit the Hopfield energy function from our previous work:
\bea
\label{eqn:H_entmax}
\calH(\bx)=-\Phi^\star\(\beta \bm{\bm{\Xi}}^\sT \bx\) +\half \Braket{\bx,\bx},
\eea
with $\Phi^\star(\cdot) \coloneqq \int\dd\bz\; \alpha$-entmax$(\bz)$ by Danskin's theorem, where $\alpha$-entmax is defined for $\bz \in \R^M$.
\begin{lemma}[Variational form of $\alpha$-entmax \cite{peters2019sparse}]
\bea
\text{$\alpha$-entmax} \coloneqq \argmax_{\bp \in \Delta^M} \[\bp^\sT z+\Phi^{\alpha}(\bp)\],
\eea
where $\Phi^{\alpha}(\bp)=\frac{1}{\alpha(\alpha-1)}\sum^M_{\mu=1}p_\mu-p_\mu^\alpha$ is the Tsallis entropic regularizer.
\end{lemma}
\begin{lemma}[Closed-form of $\alpha$-entmax]
For $\bz \in \R^M$, the $\alpha$-entmax transformation can be defined as
\bea
\label{eqn:}
\text{$\alpha$-entmax}=[(\alpha-1)\bz-\tau(\bz)]^{\frac{1}{\alpha-1}}
\eea
where we denote $[t]_{+}\coloneqq \max\{t,0\}$, and $\tau$ is the unique function $\R^M \to \R$ such that $\sum^M_{\mu=1}[(\alpha-1)\bz-\tau(\bz)]^{\frac{1}{\alpha-1}}$ satisfies the probability distribution.
\end{lemma}
Since the computation of $\alpha$-entmax in closed form relies on the choice of $\alpha$, we will discuss these special cases, i.e. 1-entmax (Softmax), 1.5-entmax and 2-entmax (Sparsemax), to analyze the impact of sparsity on modern Hopfield model.
\begin{lemma}[Danskin's Theorem]
For $\Phi$ being strictly convex, we have
\bea
\label{eqn:danskin}
\grad \Phi^\star (\bz)
=
\argmax_{\bp\in \Delta^M}\[\Braket{\bz,\bp}-\Phi^\alpha(\bp)\]
=
\text{$\alpha$-entmax},
\eea
and it can be rewritten in the indefinite integral form:
\bea
\Phi^\star(\bz)=\text{$\int \alpha$-entmax}.
\eea
\end{lemma}
\begin{lemma}[Generalized retrieval dynamics]
Denote $t$ as the iteration step. The retrieval dynamics
\bea
\label{def:sparse_retrieval_dyn}
\bx_{t+1}
=
\calT\(\bx_t\)\coloneqq\grad_\bx\Phi\(\beta\bm{\bm{\Xi}}^\sT \bx\)\big\vert_{\bx_{t}}
=
\bm{\bm{\Xi}} \text{$\alpha$-entmax}\(\beta\bm{\bm{\Xi}}^\sT \bx_t\)
\eea
can make the energy function decrease monotonically with respect to the increasing $t$.
\end{lemma}

\begin{definition} [Stored and Retrieved]
\label{def:stored_and_retrieved}
Assuming that every pattern $\bxi_\mu$ surrounded by a sphere $S_\mu$ with finite radius $R\coloneqq \half \Min_{\mu,\nu\in[M]}\norm{\bxi_\mu-\bxi_\nu}$, we say $\bxi_\mu$ is \textit{stored} if there exists a generalized fixed point of $\calT$, $\bx^\star_\mu \in S_\mu$, to which all limit points $\bx \in S_\mu$ converge to, and $S_\mu \cap S_\nu=\emptyset$ for $\mu \neq \nu$. 
We say $\bxi_\mu$ is $\epsilon$-\textit{retrieved} by $\calT$ with $\bx$ for an error\footnote{The retrieval error has a naive bound $\epsilon\coloneqq\Max\big\{\norm{\bx-\bxi_\mu},\norm{\bxi_\mu-\bx^\star_\mu}\big\}$ by interpolating from $\bx$ to $\bxi_\mu$.} $\epsilon$, if $\norm{\calT(\bx)-\bxi_\mu}\le \epsilon$.
\end{definition}
\begin{lemma}[Convergence of Retrieval Dynamics $\calT$]
\label{coro:convergence_sparse}
Suppose $\calH$ is given by \eqref{eqn:H_entmax} and $\calT(\bx)$ is given by \eqref{def:sparse_retrieval_dyn}.
For any sequence $\{\mathbf{x}_t\}_{t=0}^{\infty}$ defined by $\mathbf{x}_{t'+1} = \mathcal{T}(\mathbf{x}_{t'})$, all limit points of this sequence are stationary points if they are obtained by iteratively applying $\mathcal{T}$ to $\mathcal{H}$.
\end{lemma}
\begin{lemma}
Let $\bz \in \R^M$. For $1 \leq \alpha \leq \beta$, the inequality
\bea
[\text{$\alpha$-entmax}(\bz)]_\mu
\leq
[\text{$\beta$-entmax}(\bz)]_\mu
\eea
holds for all components of entmax.
\end{lemma}
\begin{proof}
For convenience, we define $\delta \geq 0$ by the difference of $\alpha$ and $\beta$
\bea
\delta=\beta-\alpha.
\eea
From the closed form of \text{$\alpha$-entmax}, we have
\bea
[\text{$\alpha$-entmax}]_\mu=[(\alpha-1)\bz_\mu-\tau(\bz)]_{+}^{\frac{1}{\alpha-1}}
\eea
Inserting the $\beta$, we obtain
\bea
[\text{$\alpha$-entmax}]_\mu=[(\beta-1-\delta)\bz_\mu-\tau(\bz)]_{+}^{\frac{1}{\beta-1-\delta}}.
\eea
Since $\delta>0$ and $\beta\geq\alpha\geq1$, the inequality
\bea
[(\beta-1-\delta)\bz_\mu-\tau(\bz)]^{\frac{1}{\beta-1-\delta}}
\geq
[(\beta-1)\bz_\mu-\tau(\bz)]^{\frac{1}{\beta-1}}
=
\text{$\beta$-entmax}
\eea
holds.

Therefore, for any given z and $\beta \geq \alpha \geq 1$, we have
\bea
[\text{$\alpha$-entmax}]_\mu
\leq
\text{$\beta$-entmax}_\mu.
\eea
\end{proof}

\begin{remark}
For $\alpha=1$ and $\alpha=2$, we have softmax and sparsemax, respectively.
Since $[\text{$\alpha$-entmax}(\bz)]_\mu
\leq
[\text{$\beta$-entmax}(\bz)]_\mu$ for $1\le \alpha\le \beta$ and  for all $\mu\in[M]$, 

\end{remark}

\begin{theorem}[Retrieval Error]
\label{coro:eps_sparse_dense}
Let $\calT_{\text{Dense}}$ be the retrieval dynamics of the dense modern Hopfield model \cite{ramsauer2020hopfield}.
It holds
\bea
\norm{\calT(\bx)-\bxi_\mu} 
\leq
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
\le  2m(M-1) \exp{-\beta \(\Braket{\bxi_\mu,\bx}-\Max_{\nu\in[M]}\Braket{\bxi_\mu,\bxi_\nu}\)}.
\eea
for all $\bx\in S_\mu$.
\end{theorem}

\begin{proof}
We observe
\begin{align}
&\norm{\calT(\bx)-\bxi_\mu}-\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}\nonumber\\
&=\norm{\sum_{\nu=1}^{\kappa} \bxi_\nu \[\text{$(\alpha+\delta)$-entmax}\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi_\mu}
-\norm{\sum_{\nu=1}^{\kappa} \bxi_\nu \[\text{$\alpha$-entmax}\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi_\mu}\\
&\leq
\norm{\sum^{\kappa}_{\nu=1}\[\text{$(\alpha+\delta)$-entmax}(\beta\bm{\Xi}^\sT \bx)\]_\nu\bxi_\nu }-
\norm{\sum^{\kappa}_{\nu=1} \[\text{$\alpha$-entmax}\(\beta \bm{\Xi}^\sT \bx\)\]_\nu \bxi_\nu}\leq 0,
\end{align}
which gives
\bea
\label{eqn:eps_sparse_dense}
\norm{\calT(\bx)-\bxi_\mu} 
&\leq& 
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}.
\eea
\end{proof}
Intuitively, the larger sparsity leads the lower retrieval error.

\begin{theorem}
Let $\delta\coloneqq \norm{\calT_{\text{Dense}}-\bxi_\mu}-\norm{\calT-\bxi_\mu}$.
The {well-separation} condition can be expressed as
$
\Delta_\mu \ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R+\delta})+2mR
$, which reduces to that of the dense Hopfield model when $\delta=0$.
\end{theorem}

==> additional_exp_table.tex <==
\begin{table*}[ht]
\centering
\caption{Additional Datasets: Categorical Classification}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
   Dataset ID &             BiSHop &     FT Transformer & GradientBoostingTree &       MLP & RandomForest &    Resnet &     SAINT &            XGBoost \\
\midrule
       361110 &          82.85 (6) &           83.2 (5) &            88.15 (2) & 82.42 (8) &    87.69 (3) & 82.65 (7) & 83.23 (4) & \textbf{88.61 (1)} \\
       361111 &          61.07 (4) &           60.0 (7) &            64.67 (3) & 60.54 (6) &    66.21 (2) & 59.97 (8) & 60.56 (5) & \textbf{66.85 (1)} \\
       361113 &          82.96 (8) &          85.93 (2) &            85.43 (4) & 83.32 (7) &    85.86 (3) & 83.96 (6) & 85.33 (5) & \textbf{86.58 (1)} \\
       361282 & \textbf{66.08 (1)} &          65.63 (4) &            65.76 (2) & 65.32 (7) &    65.53 (5) & 65.23 (8) & 65.52 (6) &           65.7 (3) \\
       361283 & \textbf{72.69 (1)} &           71.9 (5) &            72.09 (3) & 71.41 (7) &    72.13 (2) &  71.4 (8) &  71.9 (5) &          72.08 (4) \\
       361285 &          76.54 (4) & \textbf{77.09 (1)} &            76.31 (5) & 75.59 (8) &    76.13 (6) & 76.09 (7) & 76.69 (3) &          76.89 (2) \\
       361286 &  \textbf{69.8 (1)} &          68.97 (4) &            68.62 (6) & 69.06 (2) &    68.49 (7) &  69.0 (3) & 68.87 (5) &           68.2 (8) \\
\midrule
Average Score &              73.14 &              73.25 &                74.43 &     72.52 &        74.58 &     72.61 &     73.16 &              74.99 \\
 Average Rank &               3.57 &                4.0 &                 3.57 &      6.43 &          4.0 &      6.71 &      4.71 &               2.86 \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Additional Datasets: Numerical Classification}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
   Dataset ID &             BiSHop & FT Transformer & GradientBoostingTree &       MLP &       RandomForest &    Resnet &              SAINT &            XGBoost \\
\midrule
       361055 & \textbf{78.29 (1)} &      77.73 (2) &            77.52 (4) & 77.41 (5) &          76.35 (7) & 77.53 (3) &          77.41 (5) &          75.91 (8) \\
       361060 &           80.9 (7) &      81.95 (5) &            86.58 (2) & 80.89 (8) &          86.27 (3) & 81.16 (6) &          81.97 (4) &  \textbf{86.9 (1)} \\
       361061 &          76.91 (8) &      80.58 (5) &            81.61 (3) & 78.06 (7) &  \textbf{82.8 (1)} &  79.7 (6) &           80.6 (4) &          81.79 (2) \\
       361062 & \textbf{98.82 (1)} &       98.5 (2) &            98.16 (6) &  94.7 (8) &          98.24 (4) & 95.22 (7) &          98.21 (5) &          98.35 (3) \\
       361063 &          88.53 (4) &      88.59 (3) &            88.53 (4) & 88.06 (8) &          88.23 (6) & 88.14 (7) &          88.82 (2) & \textbf{88.83 (1)} \\
       361065 & \textbf{86.32 (1)} &      86.09 (4) &            85.79 (6) &  85.6 (7) &          85.55 (8) &  86.3 (2) &          86.04 (5) &          86.19 (3) \\
       361066 &          80.13 (4) &       80.2 (3) &            80.54 (2) & 79.48 (7) &          80.05 (5) & 79.31 (8) &          79.88 (6) & \textbf{80.62 (1)} \\
       361068 &          92.85 (7) &      93.51 (4) &            93.44 (6) & 93.45 (5) &          92.72 (8) & 93.67 (3) & \textbf{93.81 (1)} &          93.72 (2) \\
       361069 &          68.23 (8) &      70.61 (5) &            71.04 (2) & 68.97 (7) &          70.93 (3) & 69.48 (6) &          70.82 (4) & \textbf{71.37 (1)} \\
       361070 &          59.22 (5) &      59.18 (6) &            63.71 (3) & 58.89 (7) &          65.17 (2) & 58.75 (8) &          59.29 (4) & \textbf{65.77 (1)} \\
       361273 & \textbf{60.76 (1)} &      60.57 (4) &            60.53 (6) &  60.5 (7) &          60.49 (8) & 60.54 (5) &          60.59 (3) &          60.67 (2) \\
       361274 &          75.34 (7) &      76.83 (5) &            77.47 (2) & 74.57 (8) &           77.3 (3) & 75.37 (6) &          77.12 (4) & \textbf{78.03 (1)} \\
       361275 &            0.0 (8) &      71.84 (5) &            71.96 (3) & 71.34 (6) &          72.06 (2) & 71.34 (6) &          71.93 (4) & \textbf{72.07 (1)} \\
       361276 &            0.0 (8) &      75.82 (7) &            78.59 (3) &  76.7 (6) & \textbf{79.86 (1)} & 77.06 (4) &          76.87 (5) &          79.31 (2) \\
       361277 &            0.0 (8) &      89.31 (4) &            89.84 (2) & 87.24 (7) &          89.36 (3) & 87.92 (6) &          88.72 (5) & \textbf{90.35 (1)} \\
       361278 & \textbf{73.05 (1)} &      72.67 (2) &            72.35 (6) &  72.4 (4) &           72.1 (8) & 72.41 (3) &          72.37 (5) &          72.16 (7) \\
\midrule
Average Score &              63.71 &           79.0 &                79.85 &     78.02 &              79.84 &     78.37 &              79.03 &              80.13 \\
 Average Rank &               4.94 &           4.12 &                 3.75 &      6.69 &                4.5 &      5.38 &               4.12 &               2.31 \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Additional Datasets: Categorical Regression}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
   Dataset ID &             BiSHop & FT Transformer & GradientBoostingTree &                MLP &       RandomForest &            Resnet &              SAINT &            XGBoost \\
\midrule
       361093 & \textbf{98.98 (1)} &      98.06 (6) &            98.34 (3) &          98.07 (5) &          98.25 (4) &         98.04 (7) &          97.77 (8) &          98.42 (2) \\
       361094 &          99.98 (6) &      99.99 (4) &   \textbf{100.0 (1)} &          99.99 (4) & \textbf{100.0 (1)} &         99.97 (8) &          99.98 (6) & \textbf{100.0 (1)} \\
       361096 &          98.57 (8) &      98.97 (3) &            98.99 (2) &          98.77 (6) &          98.82 (5) &         98.88 (4) &          98.67 (7) & \textbf{99.11 (1)} \\
       361097 &            0.0 (8) &      56.63 (5) &            57.76 (3) &          55.91 (7) &          57.81 (2) &         57.29 (4) &          56.45 (6) & \textbf{57.87 (1)} \\
       361098 &          97.99 (8) &      99.68 (3) &            99.64 (5) &          99.68 (3) &          99.32 (6) &         99.69 (2) &           99.3 (7) &  \textbf{99.8 (1)} \\
       361099 &          94.12 (3) &      94.09 (4) &            94.26 (2) &          93.71 (6) &          93.69 (8) &         93.71 (6) &          93.75 (5) & \textbf{94.77 (1)} \\
       361101 &          49.33 (6) &      52.87 (4) &            58.56 (2) &          47.44 (7) &          58.42 (3) &         49.75 (5) &          46.31 (8) & \textbf{59.13 (1)} \\
       361102 &          83.35 (8) &      89.34 (2) &            89.28 (3) &          87.57 (6) &          87.53 (7) &         88.52 (4) &          88.36 (5) & \textbf{89.77 (1)} \\
       361103 &           63.2 (8) &      67.02 (4) &            68.57 (2) &          65.99 (7) &          67.47 (3) &         66.12 (5) &          66.02 (6) & \textbf{69.14 (1)} \\
       361104 &          99.94 (7) &      99.97 (5) &   \textbf{99.98 (1)} & \textbf{99.98 (1)} & \textbf{99.98 (1)} &         99.96 (6) &           99.9 (8) & \textbf{99.98 (1)} \\
       361287 &          -2.82 (8) &       5.33 (5) &             5.34 (4) &           4.15 (7) &  \textbf{7.36 (1)} &          5.06 (6) &           6.05 (3) &           6.94 (2) \\
       361288 &          57.96 (3) &      57.48 (4) &            55.75 (7) &          58.03 (2) &          55.79 (6) & \textbf{58.3 (1)} &          57.09 (5) &          55.75 (7) \\
       361289 &          10.91 (8) &      18.01 (6) &   \textbf{18.65 (1)} &          17.23 (7) &          18.28 (3) &         18.05 (5) &          18.22 (4) &          18.55 (2) \\
       361291 &           1.45 (8) &       6.88 (4) &              7.5 (3) &           6.26 (6) &           7.67 (2) &          6.09 (7) &           6.72 (5) &  \textbf{7.84 (1)} \\
       361292 &          50.96 (7) &      52.01 (4) &            53.04 (2) &          51.58 (5) &           49.7 (8) &         51.41 (6) &           52.6 (3) & \textbf{53.65 (1)} \\
       361293 &          -8.96 (8) &       4.67 (3) &    \textbf{4.86 (1)} &           4.17 (7) &           4.58 (4) &           4.2 (6) &           4.54 (5) &           4.85 (2) \\
       361294 &          96.76 (8) &      97.93 (3) &            97.94 (2) &          97.92 (5) &          97.88 (7) &         97.93 (3) & \textbf{97.96 (1)} &          97.89 (6) \\
\midrule
Average Score &              58.34 &          64.64 &                 65.2 &              63.91 &              64.86 &             64.29 &               64.1 &               65.5 \\
 Average Rank &               6.65 &           4.06 &                 2.59 &               5.35 &               4.18 &               5.0 &               5.41 &               1.88 \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Additional Datasets: Numerical Regression}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
   Dataset ID &             BiSHop &     FT Transformer & GradientBoostingTree &                MLP &      RandomForest &    Resnet &              SAINT &            XGBoost \\
\midrule
       361072 &           96.9 (8) &          98.48 (4) &            98.61 (2) &          97.91 (7) &         98.26 (5) & 98.26 (5) &          98.51 (3) & \textbf{98.62 (1)} \\
       361073 &          99.49 (3) & \textbf{99.51 (1)} &             99.0 (5) &          97.31 (7) &         98.67 (6) & 96.19 (8) & \textbf{99.51 (1)} &          99.15 (4) \\
       361074 &          87.65 (6) &          91.83 (2) &            85.07 (7) &          91.81 (3) &          83.3 (8) & 91.56 (4) & \textbf{91.86 (1)} &          90.76 (5) \\
       361076 &          36.62 (7) &          37.15 (6) &            47.74 (3) &          39.61 (4) &         48.07 (2) & 38.21 (5) &          36.32 (8) & \textbf{50.06 (1)} \\
       361077 &           82.4 (5) &          73.28 (6) &   \textbf{83.97 (1)} &          83.72 (2) &         83.72 (2) & 71.85 (7) &           70.1 (8) &          83.66 (4) \\
       361078 &          76.91 (8) &          83.52 (3) &            83.95 (2) &          80.97 (7) &          82.7 (5) &  83.1 (4) &          81.39 (6) & \textbf{85.22 (1)} \\
       361079 & \textbf{60.76 (1)} &          53.09 (4) &            57.45 (2) &          48.62 (7) &         50.16 (6) & 51.77 (5) &          46.79 (8) &          55.42 (3) \\
       361080 &          93.45 (8) &          94.36 (5) &            94.52 (2) &          94.41 (4) &         93.94 (7) & 94.45 (3) &          94.22 (6) & \textbf{94.56 (1)} \\
       361081 &          98.67 (8) &          99.69 (2) &            99.65 (4) &          99.52 (5) &         99.31 (7) & 99.67 (3) &          99.38 (6) & \textbf{99.76 (1)} \\
       361082 &          65.32 (8) &           68.1 (4) &            69.23 (2) &          67.71 (5) &          67.2 (6) & 67.18 (7) &          68.16 (3) & \textbf{69.61 (1)} \\
       361083 &          48.65 (5) &          49.87 (4) &            55.27 (2) &          46.79 (8) &          54.6 (3) &  48.2 (6) &          47.13 (7) & \textbf{55.37 (1)} \\
       361084 &          80.45 (8) &           88.1 (2) &             88.0 (3) &          85.72 (7) &         86.89 (5) &  86.8 (6) &          87.31 (4) & \textbf{88.92 (1)} \\
       361085 &          81.71 (6) &          81.01 (7) &             82.1 (5) &          86.83 (2) &         84.39 (4) & 85.43 (3) &          78.59 (8) & \textbf{86.87 (1)} \\
       361086 &          95.14 (8) &          97.93 (2) &   \textbf{97.94 (1)} &          97.91 (4) &         97.68 (7) & 97.93 (2) &          97.88 (5) &          97.88 (5) \\
       361087 &          84.79 (8) &          92.59 (2) &            92.57 (3) &          90.91 (7) &         91.41 (6) &  91.7 (4) &          91.58 (5) & \textbf{93.66 (1)} \\
       361088 &          87.98 (8) &          89.03 (7) &            90.32 (2) &          89.65 (4) &         90.11 (3) & 89.53 (5) &          89.09 (6) & \textbf{91.06 (1)} \\
       361279 &           0.59 (8) &           5.35 (5) &             5.57 (4) &           2.23 (7) & \textbf{9.39 (1)} &  4.28 (6) &           5.95 (3) &           8.29 (2) \\
       361280 &           56.9 (4) &          57.48 (3) &            54.87 (8) & \textbf{58.46 (1)} &         55.27 (7) & 57.81 (2) &          56.84 (5) &          55.49 (6) \\
       361281 &          -1.26 (8) &           2.11 (5) &             2.77 (3) &           1.51 (6) & \textbf{3.15 (1)} &  1.29 (7) &           2.21 (4) &           3.04 (2) \\
\midrule
Average Score &              70.16 &              71.71 &                73.08 &              71.66 &             72.54 &     71.33 &              70.67 &              74.07 \\
 Average Rank &               6.58 &               3.89 &                 3.21 &               5.11 &              4.79 &      4.84 &               5.11 &               2.21 \\
\bottomrule
\end{tabular}
}
\end{table*}



==> math_commands.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\numberwithin{equation}{section}
\usepackage{slashed}
\usepackage{braket}
\usepackage{enumitem}
\usepackage[bottom]{footmisc}
\usepackage{cite}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{subfig}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{natbib}
\usepackage{mdframed}

\usepackage{CJK}
\newcommand{\zh}[1]{\begin{CJK}{UTF8}{bsmi}\normalfont\small #1\end{CJK}} %
\newcommand{\zhs}[1]{\begin{CJK}{UTF8}{gbsn}\normalfont \small#1\end{CJK}}%

\usepackage[linesnumbered,ruled]{algorithm2e}
\SetKwComment{Comment}{/* }{ */}
\SetKwInput{kwInit}{Initialization}
\SetKwRepeat{Do}{do}{while}%


\newenvironment{claim}{  \begin{mdframed}[linecolor=black!0,backgroundcolor=black!10]\noindent%
		\ignorespaces}{\end{mdframed}}

\let\originalfigure=\figure
\let\endoriginalfigure=\endfigure

\renewenvironment{figure}[1][]{
  \begin{originalfigure}[#1]
    \begin{mdframed}[linecolor=black!0,backgroundcolor=black!1]
}{
    \end{mdframed}
  \end{originalfigure}
}

\newcommand{\comment}[1]{\textcolor{red}{[#1]}}

\def\half{{\frac{1}{2}}}
\def\sub{\scriptscriptstyle}
\def\ip{${\mathscr I}^+$}
\def\e{{\epsilon}}
\def\cs{${\cal S}$}
\def\S{\Sigma }
\def\s{\sigma }
\def\sz{\sigma^{0} }
\def\Psz{\Psi^{0} }
\def\p{\partial}
\def\cT{8\pi G_N {\mathcal T}}
\def\0{{(0)}}
\def\1{{(1)}}
\def\2{{(2)}}
\def\cL{{\cal L}}
\def\co{{\cal O}}\def\cv{{\cal V}}
\def\n{\nabla}
\def\ci{{\mathscr I}}
\def\ipp{${\mathscr I}^+_+$}
\def\<{\langle }
\def\>{\rangle }
\def\bw{{\bar w}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\g}{\gamma} 
\newcommand{\G}{\Gamma}
\newcommand{\m}{\mu}
\newcommand{\oG}{\omega}
\newcommand{\OG}{\Omega}
\newcommand{\SG}{\Sigma}
\newcommand{\sG}{\sigma}
\newcommand{\LG}{\Lambda}
\newcommand{\lG}{\lambda}
\newcommand{\tG}{\theta}
\newcommand{\TG}{\Theta}

\newcommand*\rfrac[2]{{}^{#1}\!/_{#2}}

\newcommand{\pa}{\partial}

\newcommand{\hcite}[1]{$\text{ }$\cite{#1}}
\usepackage{slashed}

\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}

\usepackage{dashbox}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{arydshln}
\definecolor{lightyellow}{rgb}{1.0, 0.95, 0.7}
\definecolor{Blue}{rgb}{0.0, 0.4, 1.0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{darkgreen}{rgb}{0.,0.6,0.}
\newcommand*{\red}[1]{\textcolor{red}{#1}}
\newcommand*{\Blue}[1]{\textcolor{Blue}{#1}}
\newcommand*{\blue}[1]{\textcolor{blue}{#1}}
\newcommand*{\green}[1]{\textcolor{darkgreen}{#1}}
\newcommand*{\black}[1]{\textcolor{black}{#1}}

\definecolor{colorA}{rgb}{1,0,0}
\definecolor{colorB}{rgb}{0,0.3,1}
\definecolor{colorC}{rgb}{0.9,0.8,0.2}
\definecolor{colorD}{rgb}{0,0.65,0}
\definecolor{lesslightgray}{rgb}{0.5,0.5,0.5}

\newcommand*{\colorA}[1]{\textcolor{colorA}{#1}}
\newcommand*{\colorB}[1]{\textcolor{colorB}{#1}}
\newcommand*{\colorC}[1]{\textcolor{colorC}{#1}}
\newcommand*{\colorD}[1]{\textcolor{colorD}{#1}}
\definecolor{light-gray}{gray}{0.95}
\newcommand{\code}[1]{\colorbox{light-gray}{\footnotesize\texttt{#1}}}

\let\tilde\widetilde
\let\hat\widehat

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}


\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\br}{\bm{r}}
\newcommand{\bq}{\bm{q}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\Max}{\mathop{ \rm Max}}
\newcommand{\Min}{\mathop{\rm Min}}
\newcommand{\Maxt}{\underset{\theta}{\Max}}
\newcommand{\Mint}{\underset{\theta}{\Min}}
\newcommand{\ArgMax}{{\rm ArgMax}}

\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}

\newcommand{\sH}{\mathsf{H}}
\newcommand{\sT}{ \mathsf{T} }

\newcommand{\sR}{\mathsf{R}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sX}{\mathsf{X}}

\def\P{\mathbb{P}}
\newcommand{\E}{\mathop{\mathbb{E}}}
\def\I{\mathcal{I}}
\def\p{\partial }
\let\cite\citep 

\newcommand{\sumN}{\sum_{i=1}^N}
\newcommand{\sumK}{\sum_{k=1}^K}
\newcommand{\sumq}{\sum_{k=1}^q}
\newcommand{\summ}{\sum_{i=1}^m}
\newcommand{\sumn}{\sum_{i=1}^n}
\newcommand{\sumd}{\sum_{i=1}^d}
\newcommand{\sumT}{\sum_{t=1}^T}
\newcommand{\sumX}{\sum_{\{\bX\}}}
\newcommand{\gradt}{\nabla_\theta}


\usepackage{amsthm}
\usepackage{nicefrac}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}[section]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}



\numberwithin{equation}{section}
\numberwithin{theorem}{section}
\newcommand{\draftpara}[1]{\paragraph{\green{#1.}}}

\usepackage{lipsum}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand*{\annot}[1]{\tag*{\footnotesize\textcolor{black!50}{#1}}}


\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
    \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
    \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
    \ifdim\ht0=\ht2 #3\else #2\fi
}
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
    \begingroup
    \def\mathaccent##1##2{%
        \let\mathaccent\save@mathaccent
        \if#32 \let\macc@nucleus\first@char \fi
        \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
        \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
        \dimen@\wd\tw@
        \advance\dimen@-\wd\z@
        \divide\dimen@ 3
        \@tempdima\wd\tw@
        \advance\@tempdima-\scriptspace
        \divide\@tempdima 10
        \advance\dimen@-\@tempdima
        \ifdim\dimen@>\z@ \dimen@0pt\fi
        \rel@kern{0.6}\kern-\dimen@
        \if#31
        \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
        \advance\dimen@0.4\dimexpr\macc@kerna
        \let\final@kern#2%
        \ifdim\dimen@<\z@ \let\final@kern1\fi
        \if\final@kern1 \kern-\dimen@\fi
        \else
        \overline{\rel@kern{-0.6}\kern\dimen@#1}%
        \fi
    }%
    \macc@depth\@ne
    \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
    \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
    \macc@set@skewchar\relax
    \let\mathaccentV\macc@nested@a
    \if#31
    \macc@nested@a\relax111{#1}%
    \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
    \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
    \fi
    \endgroup
    }
\makeatother
\let\bar\widebar


